Keypoint-based Stereophotoclinometry for Characterizing and Navigating Small Bodies: A Factor Graph Approach

This paper proposes the incorporation of techniques from stereophotoclinometry (SPC) into a keypoint-based structure-from-motion (SfM) system to estimate the surface normal and albedo at detected landmarks to improve autonomous surface and shape characterization of small celestial bodies from in-situ imagery. In contrast to the current state-of-the-practice method for small body shape reconstruction, i.e., SPC, which relies on human-in-the-loop verification and high-fidelity a priori information to achieve accurate results, we forego the expensive maplet estimation step and instead leverage dense keypoint measurements and correspondences from an autonomous keypoint detection and matching method based on deep learning to provide the necessary photogrammetric constraints. Moreover, we develop a factor graph-based approach allowing for simultaneous optimization of the spacecraft's pose, landmark positions, Sun-relative direction, and surface normals and albedos via fusion of Sun sensor measurements and image keypoint measurements. The proposed framework is validated on real imagery of the Cornelia crater on Asteroid 4 Vesta, along with pose estimation and mapping comparison against an SPC reconstruction, where we demonstrate precise alignment to the SPC solution without relying on any a priori camera pose and topography information or humans-in-the-loop

==> figs/filter-results.tex <==
\begin{tabular}{@{}lrrrrrcrrrrr@{}}\toprule
 & \multicolumn{5}{c}{With filtering} && \multicolumn{5}{c}{Without filtering} \\
\cmidrule{2-6} \cmidrule{8-12}
$\sigma_\mathbf{x}$ (pixels) & $\delta\ell\ \left(\text{m}\right)$ & $\|\delta\vvec{r}\|\ \left(\text{m}\right)$ & $\|\delta\vvec{\kappa}\|\ \left(^{\circ}\right)$ & $\delta\epsilon\ \left(^{\circ}\right)$ & $\delta a$ && $\delta\ell\ \left(\text{m}\right)$ & $\|\delta\vvec{r}\|\ \left(\text{m}\right)$ & $\|\delta\vvec{\kappa}\|\ \left(^{\circ}\right)$ & $\delta\epsilon\ \left(^{\circ}\right)$ & $\delta a$ \\ 
\midrule
1 & $3.0022$ &  $31.9866$ & $0.2294$ &  $5.3082$ ($35.3347$) & $0.0106$ && $1.9585$ &  $39.7637$ & $0.3025$ &  $5.0666$ ($35.2616$) & $0.0149$ \\
3 & $4.0807$ & $115.0922$ & $0.9678$ & $11.6405$ ($35.3347$) & $0.0226$ && $3.5869$ & $131.7686$ & $1.0289$ & $10.7963$ ($35.2939$) & $0.0199$ \\
5 & $3.2426$ & $215.5698$ & $1.6743$ & $13.4507$ ($35.3347$) & $0.0248$ && $3.5442$ & $189.8494$ & $1.4984$ & $13.5536$ ($35.3020$) & $0.0221$ \\
\bottomrule
\end{tabular}

==> figs/spc-results-500.tex <==
\begin{tabular}{lrrrcrrrcrrrrrr}\toprule
 & \multicolumn{3}{c}{SfM} && \multicolumn{3}{c}{SPG} && \multicolumn{5}{c}{SPC} \\
\cmidrule{2-4} \cmidrule{6-8} \cmidrule{10-15}
Model & $\delta\ell\ \left[\text{km}\right]$ & $\|\delta\vvec{r}\|\ \left[\text{km}\right]$ & $\|\delta\bm{\kappa}\|\ \left[^{\circ}\right]$ && $\delta\ell\ \left[\text{km}\right]$ & $\|\delta\vvec{r}\|\ \left[\text{km}\right]$ & $\|\delta\bm{\kappa}\|\ \left[^{\circ}\right]$ && $\delta\ell\ \left[\text{km}\right]$ & $\|\delta\vvec{r}\|\ \left[\text{km}\right]$ & $\|\delta\vvec{\kappa}\|\ \left[^{\circ}\right]$ & $\delta\epsilon_\mathrm{s}\ \left[^{\circ}\right]$ & $\delta\epsilon_\mathrm{n}\ \left[^{\circ}\right]$ & $\delta a\ \left[\%\right]$ \\ 
\midrule
\rowcolor[gray]{0.9}
L-Lambert                    & & & && & & && & & & & & \\
$\quad+$ $\lambda_k, \xi_k$  &  $TBD$ &  $TBD$ & $TBD$ && $TBD$ &  --- & --- && $TBD$ &  $TBD$ & $TBD$ &  $TBD$ & $TBD$ & $TBD$\\
\rowcolor[gray]{0.9}
$\quad+$ $f_\mathrm{smooth}$ &  $TBD$ &  $TBD$ & $TBD$ && $TBD$ &  --- & --- && $TBD$ &  $TBD$ & $TBD$ &  $TBD$ & $TBD$ & $TBD$\\
$\quad+$ I/F images          &  $0.0288$ &  $3.9530$ & $0.3470$ && $0.0471$ &  --- & --- && $0.0901$ & $4.4139$ & $0.3875$ & $3.1805$ &  $9.17$ & $6.04$ \\
\midrule
\rowcolor[gray]{0.9}
Sch\"{o}der                  & & & && & & && & & & & & \\
$\quad+$ $\lambda_k, \xi_k$  &  $0.0059$ &  $0.1030$ & $0.0088$ && $0.0389$ &  --- & --- && $0.0913$ & $0.9135$ & $0.0791$ & $0.2167$ & $14.08$ & $6.51$ \\
\rowcolor[gray]{0.9}
$\quad+$ $f_\mathrm{smooth}$ &  $0.0047$ &  $0.2380$ & $0.0209$ && $0.0389$ &  --- & --- && $0.0911$ & $0.9453$ & $0.0824$ & $0.2715$ &  $4.89$ & $3.84$ \\
$\quad+$ I/F images          &  $0.0042$ &  $0.2536$ & $0.0219$ && $0.0387$ &  --- & --- && $0.0908$ & $0.9123$ & $0.0796$ & $0.3534$ &  $4.66$ & $3.76$ \\
\bottomrule
\end{tabular}

==> text/recycle_bin.tex <==
% \begin{figure}[p]
% \centering
% \input{figs/reconstruction-results-llambert}
% \caption{Quantitative comparison between our solution and the SPC solutions with respect to landmark error, normal error, and relative albedo error for the Lunar-Lambert~\cite{} reflectance function.}
% \label{fig:reconstruction-results-llambert}
% \end{figure}

% \begin{figure}[p]
% \centering
% \input{figs/reconstruction-results-schroder}
% \caption{Quantitative comparison between our solution and the SPC solutions with respect to landmark error, normal error, and relative albedo error for the Schr\"{o}der~\cite{} reflectance function.}
% \label{fig:reconstruction-results-schroder}
% \end{figure}


% \begin{figure}[p]
% \centering
% \input{figs/spc-comparison-llambert}
% \caption{Quantitative comparison between our solution and the SPC solutions with respect to landmark error, normal error, and relative albedo error for the Lunar Lambert~\cite{} reflectance function.}
% \label{fig:spc-comparison-llambert}
% \end{figure}

% \begin{figure}[p]
% \centering
% \input{figs/spc-comparison-schroeder}
% \caption{Quantitative comparison between our solution and the SPC solutions with respect to landmark error, normal error, and relative albedo error for the Schr\"{o}der~\cite{} reflectance function.}
% \label{fig:spc-comparison-schroeder}
% \end{figure}


\begin{figure}[p]
\centering
\input{figs/spc-sfm-spg-comparison-llambert}
\caption{Quantitative comparison between our solution and the SPC, SfM, and SPG solutions with respect to landmark error.}
\label{fig:reconstruction-results-llambert}
\end{figure}

\begin{figure}[p]
\centering
\input{figs/spc-sfm-spg-comparison-schroder}
\caption{Quantitative comparison between our solution and the SPC, SfM, and SPG solutions with respect to landmark error.}
\label{fig:reconstruction-results-schroder}
\end{figure}
